F\'isica Estad\'istica: teor\'ia, ejemplos trabajados, modelos y simulaciones

In this book, we study Statistical Physics under conditions of thermodynamic equilibrium, starting from the definition of statistical ensembles. The book is divided into five chapters: First, a brief introduction to statistical methods. Second, the statistical description of isolated systems, corresponding to microcanonical ensembles. Third, the statistical description of systems in contact with a heat reservoir at a constant temperature T, known as the canonical ensemble. Fourth, the description of systems in contact with a heat reservoir at temperature T and with a constant chemical potential {\mu}; the grand canonical ensemble. And finally, quantum statistics. In each chapter, a theoretical description, worked examples, links to simulations (see GitHub repository: https://github.com/davidalejandromiranda/StatisticalPhysics) and discussions on recent scientific reports will be presented so readers can complement their studies.

==> author.tex <==
%%

\chapter{Acerca de los autores}

\textbf{David A. Miranda} es profesor Titular de la Escuela de Física de la Universidad Industrial de Santander, UIS, Bucaramanga, Colombia, donde se encuentra vinculado desde 2006. Su formación a nivel de pregrado corresponde con ingeniero electrónico (2003) y físico (2004). A nivel de posgrado, obtuvo una maestría en ingeniería (2005), mientras que su doctorado fue obtenido en química aplicada (2011). Sus campos generales de interés en investigación son la fisicoquímica, biofisicoquímica y educación (\href{https://orcid.org/0000-0003-3130-3314}{orcid.org/0000-0003-3130-3314}), centrados en entender la biofisicoquímica del cáncer, el modelado mecánico cuántico de sistemas mesoscópicos y cómo mejorar la experiencia de aprendizaje y enseñanza de los estudiantes mediante el uso de metodologías de aprendizaje y tecnologías de la información. Tiene habilidades avanzadas en el desarrollo de software que incluyen Python, Swift (iOS) y MATLAB.

%David A. Miranda is a professor of physics at Universidad Industrial de Santander, UIS, Bucaramanga, Colombia. He has a bachelor's degree in both electronic engineering (2003) and physics (2004). He obtained a master's degree in engineering (2005), whereas his Ph.D. degree was obtained in applied chemistry (2011). His general research fields of interest are in physical chemistry, biophysical chemistry and education (orcid.org/0000-0003-3130-3314), focused on understanding the biophysical chemistry of cancer, quantum mechanical modelling of mesoscopic systems and how to improve the learning and teaching experience of students by using learning methodologies and information technologies. He has advanced skills in software development that include Python, Swift (iOS) and MATLAB.

\begin{center}
    \href{https://orcid.org/0000-0003-3130-3314}{Orcid}, \href{https://scienti.minciencias.gov.co/cvlac/visualizador/generarCurriculoCv.do?cod_rh=0000446289}{CvLAc}, \href{https://publons.com/researcher/2199732/david-alejandro-miranda-mercado/}{Publons}, \href{https://scholar.google.com.co/citations?user=2pb-cFoAAAAJ&hl=en}{Google Scholar}, \href{https://expertic.uis.edu.co/david}{ExperTIC}.
\end{center}

\textbf{Carlos J. Paez} es profesor XX de la Escuela de Física de la Universidad Industrial de Santander, UIS, Bucaramanga, Colombia, donde se encuentra vinculado desde 20XX.

==> sections/S11_ch3.tex <==
\section{Caso de estudio III.6. Oscilador armónico clásico}
\index{Oscilador armónico clásico}

\section{Caso de estudio III.7. Calor específico de sólidos}
\index{Calor específico en sólidos}

<<Ley de Dulong-Petit, modelo de Einstein y modelo de Debye para el calor específico en sólidos>>

\href{https://colab.research.google.com/github/davidalejandromiranda/StatisticalPhysics/blob/main/notebooks/es_CalorEspecificoSolidos.ipynb}{Simulación III.3. Calor específico de sólidos}

\section{Caso de estudio III.8. Teoría cinética de los gases diluídos}
\index{Teoría cinética de los gases}

\section{Caso de estudio III.9. Paramagnetismo de partículas con momento angular total J}
\index{Paramagnetismo}

==> sections/S16.tex <==
% \section{Gas ideal de fermiones}
